CaPC Learning: Confidential and Private Collaborative Learning

Machine learning benefits from large training datasets, which may not always be possible to collect by any single entity, especially when using privacy-sensitive data. In many contexts, such as healthcare and finance, separate parties may wish to collaborate and learn from each other's data but are prevented from doing so due to privacy regulations. Some regulations prevent explicit sharing of data between parties by joining datasets in a central location (confidentiality). Others also limit implicit sharing of data, e.g., through model predictions (privacy). There is currently no method that enables machine learning in such a setting, where both confidentiality and privacy need to be preserved, to prevent both explicit and implicit sharing of data. Federated learning only provides confidentiality, not privacy, since gradients shared still contain private information. Differentially private learning assumes unreasonably large datasets. Furthermore, both of these learning paradigms produce a central model whose architecture was previously agreed upon by all parties rather than enabling collaborative learning where each party learns and improves their own local model. We introduce Confidential and Private Collaborative (CaPC) learning, the first method provably achieving both confidentiality and privacy in a collaborative setting. We leverage secure multi-party computation (MPC), homomorphic encryption (HE), and other techniques in combination with privately aggregated teacher models. We demonstrate how CaPC allows participants to collaborate without having to explicitly join their training sets or train a central model. Each party is able to improve the accuracy and fairness of their model, even in settings where each party has a model that performs well on their own dataset or when datasets are not IID and model architectures are heterogeneous across parties.

==> Contents/5_implement.tex <==
\section{Implementation}
\label{sec:implement}
For a single run of the protocol, we instantiate $\mathcal{P}_{i_*}$ as a client (a querying party) and each $\{\mathcal{P}_i\}_{i \ne i_*}$ acts as a server (an answering party). For ease of exposition, in most of the steps below we focus on a single server and client. 

To implement the first step of the protocol, we use the he-transformer library~\citep{he-transformer-lib} for the deep learning inference on encrypted data, which is the main bottleneck of the protocol in terms of the computational performance. 
\xiao{the following are all non-essential details of HET lib, not our code. Consider remove
The linear layers (e.g., convolution or batch normalization) are computed using homomorphic encryption (HE), while the secure multi-party computation (\smc) and garbled circuits (GC) are used to compute the non-linear layers, such as ReLU. The client stores the secret key $sk_i$, encrypts data with its public key $pk_i$, and sends the encrypted data to the server for inference. The server runs the model $\mathcal{M}_i$ on the encrypted data and outputs encrypted logits.}
\varun{1. the argument about choosing $\hat{r}_i$ -- while intuitive is not very formal; 2. if there are conditions imposed on choosing $\hat{r}_i$ -- you're not really "uniformly/randomly" sampling it}

In the second step, the server selects a random vector $\hat{\bm r}_i$ that is encrypted on the server side using the client's public key $pk$ to obtain ${\sf Enc}_{pk}(\hat{\bm r}_i)$ and subtracted from the encrypted vector of logits ${\sf Enc}_{pk}({\bm r}_i)$. The result is returned to the client that decrypts it and obtains ${\bm r}_i - \hat{\bm r}_i$. The logits are not normalized and can be arbitrary numbers. The random elements in vector $\hat{\bm r}_i$ have to be selected carefully since if all of their absolute values are smaller than the smallest logit then, in most cases, the client could perform argmax on the ${\bm r}_i - \hat{\bm r}_i$ to obtain desired results (e.g., the exact labels returned by the model $\mathcal{M}_i$). Thus, the absolute values in $\hat{\bm r}_i$ should be larger than the largest logit. Then, for a given mini-batch of examples, the client obtains ${\bm r}_i - \hat{\bm r}_i$, whose argmax is dominated by a single largest value (that we can choose arbitrary) and each example is assigned the same label. Hence, without the knowledge of $\hat{\bm r}_i$, the accuracy of the model, from the client perspective, is close to a random model, which is a desired property. To estimate the expected largest logit on the server $\mathcal{P}_{i}$, we can run all examples available in the plain text  through the model $\mathcal{M}_i$ and find a single maximum value of all the logits. 

The goal of the third step of the protocol is to compute the one-hot encoding of the result. The client and server engage again in the secure two party computation using our own implementation of the garbled circuit (GC) based on the EMP-toolkit~\citep{emp-toolkit}. The one-hot vector representation is a secret that is shared among the client and server. 

In the fourth step, the client computes the sum of all its secret shares. The CSP is a service that receives the secret shares from servers $\{\mathcal{P}_i\}_{i \ne i_*}$, computes their sum, and adds DP (Differential Privacy) noise to the output. The last step prevents the answering parties $\{\mathcal{P}_i\}_{i \ne i_*}$ from revealing any information about their private data (that models $\{\mathcal{M}_i\}_{i \ne i_*}$ were trained on).

In the final step, CSP acts as a server and engages in a secure two-party computation with the client $\mathcal{P}_{i_*}$ to compute the final argmax of the aggregated results (this is equivalent to a majority vote in ensemble methods). The final result is visible to the CSP and the client.

==> Contents/6_experiments_privacy_vs_utility.tex <==
We now study the trade-off between privacy and utility of our obtained models. Recall that we add (Gaussian or Laplacian) noise to the aggregate of predicted labels of all parties. Under the uniform setting, we choose the standard deviation, $\sigma$, by performing a (random) grid search and choosing the highest noise before a significant loss in accuracy is observed. In doing so, each query uses minimal $\varepsilon$ while maximizing utility. Figure~\ref{fig:tuning-privacy} in Appendix~\ref{sec:app:experiments} shows a sample plot for $K=250$ models.

As we vary the number of effective (virtual) parties, we can issue more queries for a given privacy budget, $\varepsilon$. In Figure~\ref{fig:acc-privacy-nr-models}, we report the accuracy gain achieved using \capc with various numbers of parties, $K$. As we have a fixed total dataset size, increasing the number of parties decreases their training data size, leading to worse performing models. These models see the largest benefit from \capc but, importantly, we always see a net improvement across all values of $K$. 
% We visualize the accuracy of models obtained with different amount of privacy budget (the $\varepsilon$ value in DP) in Figure~\ref{fig:acc-privacy-nr-models}. We measure the utility improvement (as mean accuracy) provided by \capc under uniform data distribution and homogeneous model architecture in function of privacy budget. We run the experiment using VGG like architecture of the models trained on SVHN dataset. %The higher the privacy budget (epsilon), the higher the accuracy should be. 
% We report the average accuracy of the models trained only on the private data for the zero privacy budget. For $N$ participating models, we divide the training set into $N$ parts, and train each model on its corresponding part. Thus, the setting with 300 participating models has the lowest initial average accuracy since the models are trained on the smallest amount of private data.
% The highest gain in accuracy, measured as the difference between the retrained models and the models trained only on the private data, is for the largest number of participating models, 300 in our experiments. This is because these models are the weakest, in terms of their initial accuracy, and can benefit most from additional data provided during retraining. The accuracy gain in the case of 50 participating models is much smaller, only 0.2\%. However, we already start with a very strong models and despite that can provide an increase in accuracy, especially in the cases where even small improvements are highly desired.

% For each number of participating models, we can find the amount of the privacy budget that allows us to obtain gains in accuracy. For the small number of participating models (less than 150), the best values of $\varepsilon$ are relatively small ($\le 1.0$ in our results). The privacy budget can be increased significantly when we increase the number of models. Each experimental configuration is run until the maximum privacy budget is reached. 
% \chris{we use 7 for stddev in privacy SVHN, 4 on CIFAR}\adam{Chris, it'd be great if you can you add this info in the proper text (and not only in the comment).}

% \adam{Another approach is to train the proper ResNet18 or VGG16 models on the small subsets of private data (instead of VGG6 or ResNet8) because during collaborative retraining we expect to provide much more data items and the model capacity should be large enough to be able to retrain on ultimately the whole training set.}


%\part The accuracy of retrained models obtained with different amount of privacy budget for different number of parties (and models) in \capc.
%\label{fig:acc-privacy-budget-model-nr}
\begin{figure}[htb]
\begin{minipage}{0.4\textwidth}
\centering
    % \includegraphics[width=0.7\columnwidth]{figures/grads_ratio_c_values_single_1.pdf}
    \includegraphics[width=50mm]{graphs/accuracy-vs-privacy-budget-vary-number-of-models.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{c|c|c}
        \thead{\textbf{Number of}\\\textbf{Parties, $K$}} & \thead{\textbf{Accuracy} \\ \textbf{Gain (\%)}} & \thead{\textbf{Best} \\ \textbf{$\varepsilon$}} \\
        \hline
        50 & 0.20 & 1.0 \\
        \hline
        100 & 0.67 & 1.0\\
        \hline
        150 & 0.165 & 5.5\\
        \hline
        200 & 1.26 & 3.5 \\
        \hline
        250 & 1.72 & 2.0 \\
        \hline
        300 & 3.25 & 2.5 \\
\end{tabular}
\captionof{figure}{
\textbf{Accuracy gain with \capc for varying number of effective parties, $K$.} 
% Accuracy of retrained models for different privacy budget and number of models participating in \capc.
}
\label{fig:acc-privacy-nr-models}
\end{minipage}
\end{figure}

==> Contents/experiments_backup.tex <==

\section{Experiments}

\capc aims to improve model utility of collaborating parties by providing them with new labelled data for training their respective private models. Since the \capc protocol is a structured application of techniques for confidentiality (i.e., confidential inference and secret sharing) and differential privacy (i.e.,  private aggregation)
%To ensure privacy, we use the PATE differential privacy scheme which, like any differential privacy method, will incur some loss in model utility (as a trade-off with privacy). To ensure confidentiality, we incur some computational overhead in executing this protocol. Thus, 
we consider the following three major dimensions in our experiments:
\begin{enumerate}
    \item How well does collaboration improve the accuracy of all participating parties?
    \item What requirements are there to achieve privacy and how can these be relaxed under different circumstances? What is the trade-off between the privacy provided  and the utility of \capc?
    \item What computational cost is there to ensuring confidentiality?
\end{enumerate}

\natalie{I think we may need to re-structure this whole section a bit more - it would be more concise to first describe all of our settings (uniform/non-uniform, homogeneous/heterogeneous, datasets, and the number of QPs and APs in each experiment) then we can go on to describe the metrics we are assessing. As it currently stands, we are mixing describing the settings and the metrics we are evaluating which is messy}

\subsection{Evaluation Setup}
Unless otherwise stated, we uniformly sample from the training set of the dataset in use\footnote{For SVHN dataset, we combine its original training set and extra set to get a larger training set.}, without replacement, to create disjoint datasets of equal size for each party. We select $K=50$ and $K=250$ total parties for CIFAR10 and SVHN, respectively (unless otherwise noted). We select $Q$ querying parties ($\mathcal{P}_{i_*}$) on each dataset and similarly divide the test sets to act as a private pool for each querying party. Querying parties select queries from this pool until a privacy budget of $\epsilon$ is reached. The querying parties then retrain their models using the additional labeled data (from \capc). On CIFAR10, we use a pool size of $3,000$ leaving $1,000$ data points for test evaluation. On SVHN, we use a pool size of $10,000$ leaving $16,032$ for test evaluation. We use accuracy as our test evaluation metric except for fairness experiments that use balanced accuracy (see Definition~\ref{balanced_accuracy}). Models are trained (and retrained) for $200$ epochs and a batch size of $128$, with a learning rate of $0.1$ that decays by a factor of $10$ at epochs $100$, $150$, and $180$. For ResNet models, we reduce the learning rate by a factor of 2 once their learning stagnates (for more than 10 epochs). The weight decay is set to $1e-4$ and momentum to $0.9$ (details on the architectures can be found in the appendix~\ref{subsection:architecture-details}).

\subsection{Implementation}
\label{ssec:implement}
We use the HE-transformer library with MPC (MP2ML)~\citep{he-transformer-lib}  for confidential two-party deep learning inference and the EMP~\citep{emp-toolkit} toolkit for generic two-party computation, to compute operations including $\argmax$ and $sum$ using its garbled circuits implementations. Since all logits are real numbers, we need to use statistical secret sharing where the shares are much larger than the underlying value being shared. We use the single largest logit value for each $\mathcal{M}_i$ obtained on its training set $\mathcal{D}_i$ in plain text to calculate the necessary noise. It may instead be possible to bound the maximum logit value. Due to limitations in the HE-transformer library for maximum float value in their encryption scheme, we were only able to add sufficient noise to achieve secret sharing with statistical security of $2^{-20}$. To support even stronger level of statistical security, one would need to tweak the way HE-transformer encodes real numbers. Other components of our code are already implemented to support stronger statistical security.

\todo{add pointer to old content if it is still lying around}

\todo{add datasets architectures etc even if pointer to appendix}


\subsection{Collaboration}
We first investigate the benefits of collaboration to improving model performance (Section~\ref{uniform-distribution} demonstrates improvements to accuracy).  In particular, we are focused on understanding the benefits of \capc under varying model heterogeneity (Section~\ref{uniform-distribution} demonstrates improvements to all model types) and there is increasing data distribution shift between parties (Section~\ref{non-uniform-distribution} shows improvements to accuracy but also certain fairness metrics). Our heterogeneous model study, where parties employ different model architecture to train their models $\mathcal{M}_i$, is a setting that \capc enables unlike related approaches (e.g., federated learning).



% We find in Section~\ref{uniform-distribution} that under no skew, collaborative learning can increase overall and class-specific accuracies for all models, even if models are heterogeneous. In Section~\ref{non-uniform-distribution}, we find that this remains true even under data skews between parties, which can lead to even greater benefits under fairness metrics.
% In  we find that active learning can further improve benefits and  that \capc applies even in the heterogeneous setting.
% \Chris{If there isn't space we can cut this.}

% \begin{itemize}
% \item When data distribution is similar across all parties, collaborative learning can increase model accuracy (both class-specific and mean) for all querying parties.
% \item When there is distribution drift between different parties, collaborative learning can increase both model accuracy and fairness for all querying parties.
% \end{itemize}

\subsubsection{Uniformly Sampled Private Data}
\label{uniform-distribution}



The first setting we consider is a uniform distribution of data amongst of parties---there is no data drift among parties. To this end, we take our $Q=3$ querying parties and use a random sampling strategy to choose data points (until $\epsilon=2$ and $\epsilon=20$, in SVHN and CIFAR10, respectively) to be labelled by the other $K-1$ parties.

In Figure~\ref{fig:uniform-all}, we see that there is a consistent accuracy increase across all classes and all parties, in both a homogeneous and heterogeneous setting. Interestingly, heterogeneity in the \capc setting improves the learning among all parties. Figures~\ref{fig:uniform-cifar-split},~\ref{fig:uniform-svhn-split},~and~\ref{fig:hetero-uniform-svhn-split} provide a breakdown of the benefits obtained by each querying party. In only $6.67\%$ of all cases were any class-specific accuracies degraded, but to a still net increase of overall accuracy for the model. 

% \chris{we don't fine-tune, we retrain with the new data from \capc}
% \chris{SVHN we train for 200 epoch, using 2500 examples per model (uses the extra training data) batch size is 128. we use the privacy budget of 2 for svhn and 20 for cifar10 giving around 500 samples.
% we use 50 models for cifar10 (1000 sampels per model).
% learning rate begins at 0.1 and decays by a factor 10 at 50\%, 75\%, 90\%
% weight decay and momentum are standard.
% }
 

% For CIFAR10 dataset, we set the effective number of parties to 50 and only allow the first 3 parties to pose queries. The original CIFAR10 training set is uniformly divided into 50 disjoint partitions on which each party trains their individual private model. The first 9000 samples in the original CIFAR10 test set is uniformly divided into 3 disjoint partitions (a.k.a the unlabeled sample pools of querying parties) from which each querying party selects queries. The remaining 1000 samples in the original CIFAR10 test set is used as evaluation data. 

\begin{figure}[htb]
\centering
\begin{minipage}{0.32\linewidth}
\centering
% \captionsetup{justification=centering}
\includegraphics[width=1\linewidth]{graphs/uniform-CIFA.pdf}
% \caption*{CIFAR10, \\ Homogeneous}
\end{minipage}
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{graphs/uniform-SVHN.pdf}
    % \captionsetup{justification=centering}
    % \caption*{SVHN, \\ Homogeneous}
\end{minipage}
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{graphs/heterogeneous-SVHN.pdf}
    % \captionsetup{justification=centering}
    % \caption*{SVHN, \\ Heterogeneous}
\end{minipage}
% \begin{minipage}{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{graphs/cifar10-qp1-accuracy.pdf}
% \caption{Querying party 1.}
% \end{minipage}
% \begin{minipage}{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{graphs/cifar10-qp2-accuracy.pdf}
% \caption{Querying party 2.}
% \end{minipage}
% \begin{minipage}{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{graphs/cifar10-qp3-accuracy.pdf}
% \caption{Querying party 3.}
% \end{minipage}
\caption{\textbf{Using \capc to improve each party's model performance.} We observe a mean increase of $4.09$ and of $1.92$ percentage points on CIFAR10 and SVHN, respectively, when using homogeneous models and an increase of $2.64$ with heterogeneous models; each party still sees improvements.}
\label{fig:uniform-all}
\end{figure}

% For SVHN dataset, we set the effective number of parties to 250 and only allow the first 3 parties to pose queries. The original SVHN training set and extra set are uniformly divided into 50 disjoint partitions, respectively, and each party trains their individual private model on the combination of one partition from the training set and one partition from the extra set. The first 10000 samples in the original SVHN test set is uniformly divided into 3 disjoint partitions (a.k.a the unlabeled sample pools of querying parties) from which each querying party selects queries. The remaining 16032 samples in the original SVHN test set is used as evaluation data. 
    % \chris{TODO: evaluate heterogeneous models here}


\subsubsection{Non-Uniformly Sampled Private Data}
\label{non-uniform-distribution}

\nicolas{old comment: in the presence of different participant training distributions, fairness improvements when we have imbalance between the participants (even with the participants have lots of data, they might still be able to learn about a data point in the tail of the distribution that another hospital has data for)}


In this section, we focus on understanding two types of data shifts between parties: varying size of data per class and total size of data provided. These shifts are motivated by our application scenarios: certain hospitals may specialize in specific treatments that may lead them to have a larger population compared with other hospitals. Further, some hospitals may be located in a more population-dense area and thus have more data overall. In either scenario, it is important that the parties with an advantage still gain from the collaborative setting. To analyze data skew, we now explore using the balanced accuracy (see Definition~\ref{balanced_accuracy}). To overcome pitfalls in a random sampling strategy, we now look toward active learning techniques, namely entropy and margin (see Definitions~\ref{entropy_sampling}~and~\ref{margin_sampling}).

To this end, we reuse our uniform experiments but now vary the distribution of data in the private datasets of the $K=3$ querying parties. On CIFAR10, they now have 80\% less data samples for classes `horse', `ship' and `truck'. On SVHN, they now have 90\% less data samples for classes 1 and 2. Since these classes are are under-sampled, we employ different active learning strategies (rather than just randomly sampling): we use margin and entropy sampling (see Definitions~\ref{margin_sampling}~and~\ref{entropy_sampling}). In Figure~\ref{fig:non-uniform} we see that random sampling does not in fact have a significant impact on the balanced accuracy when there is data skew between the private data of participating parties. Leveraging active learning techniques, we overcome this pitfall and achieve benefits in balanced accuracy for both datasets, because these methods more heavily sample the underrepresented classes, as shown in Figure~\ref{fig:query-amount} (see the Appendix).

\begin{figure}[htb]
\begin{minipage}{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{graphs/nonuniform-CIFA.pdf}
    % \caption*{\centering CIFAR10}
\end{minipage}
\begin{minipage}{0.49\linewidth}
    \includegraphics[width=1\linewidth]{graphs/nonuniform-SVHN.pdf}
    % \caption*{\centering SVHN}
\end{minipage}
\caption{\textbf{\capc with active learning to improve balanced accuracy given non-uniform private data.} We observe that random sampling does not significantly improve balanced accuracy but the best active learning scheme can improve the balanced accuracy by a further $2.95$ percentage-points on CIFAR10 and $0.42$ percentage-points on SVHN.}
\label{fig:non-uniform}
\end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.98\linewidth]{graphs/active-learning-imbalanced-distribution.pdf}
% \caption{
% Model accuracy obtained with different query selection strategies on CIFAR10 (left) and SVHN (right). Standard deviation is measured on all class-specific accuracy values.
% }
% \chris{should we average across 3 QP's or just show 1 QP?}
% \end{figure}

% \chris{techniques to evaluate: entropy, gap, random, k-center greedy?, @yunxiang, what is ready, what needs to be done?}

% \subsubsection{Collaboration with Heterogeneous models}\label{ssec:heterogeneous}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.98\linewidth]{graphs/heterogeneous-SVHN.pdf}
% \caption{\textbf{Model accuracy}
% }
% \end{figure}

\subsection{Privacy vs Utility}
\input{Contents/6_experiments_privacy_vs_utility}


\subsection{Adding Confidentiality}

The incorporation of confidentiality in the \capc protocol introduces two significant impacts on the trained model on which inference is completed. The inclusion of confidentiality in \capc --- in our implementation, through use of homomorphic encryption and garbled circuits --- can lead to minimal degradation in accuracy due to accumulation of error associated with these cryptographic methods across layers of the model. More notably, integration of security in inference with \capc incurs an increased computational expense. We segment the analysis of computational overhead into three parts corresponding to sequential steps in the protocol: (1) inference, (2) secret sharing between each querying and answering party, and (3) secret sharing between the querying party and the \pg. Each of these steps is analyzed in terms of Wall Clock Time in seconds to complete the step on different methods. We consider the following methods for computation of each step: base encryption, GPU with no encryption, and CPU with no encryption. 

\chris{notes: 1. can be improved by batching, we should compare with teh baseline of doing each model on a GPU (since he-transformer does cpu). I currently includen etwork time in 1. but we can separate out if needed.
2. is fixed
3. is fixed.}
\begin{table}[t]
    \begin{minipage}{0.75\linewidth}
    \centering
    \begin{tabular}{c | c | c | c}
    Method & \multicolumn{1}{|p{1.85cm}|}{\centering Forward Pass \\ (Step 1)} & \multicolumn{1}{|p{1.95cm}|}{\centering QP-AP \\ (Step 2 and 3)}  & \multicolumn{1}{|p{1.95cm}|}{\centering QP-\pg \\ (Step 4 and 5)} \\
    \toprule
    % GPU, no encryption & $15.1046 \pm 0.356$ & \\
    $poly\_modulus\_degree=8192$ & $14.22 \pm 0.11$ & \multirow{5}{*}{$0.12 \pm 0.0058$} & \multirow{5}{*}{$0.030 \pm 0.0045$}\\
    $poly\_modulus\_degree=16384$ & $29.46 \pm 2.34$ &  & \\
    $poly\_modulus\_degree=32768$ & $57.26 \pm 0.39$ &  & \\
    GPU, no encrpytion & $3.15 \pm 0.22$ & & \\
    CPU, no encryption & $0.152\pm 0.0082$ & \\
    \end{tabular}
    \caption{\textbf{Wall Clock Time (s) of various encryption methods.}}
    \end{minipage}
    % \begin{minipage}{0.5\linewidth}
    % \centering
    % \begin{tabular}{c | c | c}
    %     Forward Pass (Step 1) & QP-AP (Step 2 and 3)  & QP-\pg (Step 4 and 5) \\
    %     \toprule
        
    % \end{tabular}
    % \caption{Wall Clock Time (s)}
    % \end{minipage}
    \label{tab:confidentiality-overhead}
\end{table}





\subsection{Performance}
\label{sec:performance}
\nicolas{
%in the presence of different participant training distributions, fairness improvements when we have imbalance between the participants (even with the participants have lots of data, they might still be able to learn about a data point in the tail of the distribution that another hospital has data for)
What do we pay for confidentiality: computational and network communication overhead and accuracy if security strength increases 

- What do we pay for privacy: utility. Here we'll show we get somewhat weak guarantees but we expect the trust among hospitals does not require super low epsilon. Unclear how tight data-dependent bounds? }

The highest computational cost and most of the data movements occurs during the neural network inference using MPC for HE-transformer~\citep{he-transformer-lib}. This constitutes the first step in the \capc pipeline.
%The results reported, for instance, for Delphi~\citep{delphi} (and other such tools) present the exact amount of data moved. For example, Delphi decreased this amount substantially compared to Gazelle~\citep{gazelle}.
%In our case, 
The additional overhead when we move around the one-hot vectors in \capc is relatively small in comparison to the feature maps sent via network for ReLU or MaxPool layers that are executed via MPC.

%\natalie{the above exposition on delphi should maybe be moved to discussion - we should restrict this section solely to experiments and results, but related works and justification for use of certain tools can be moved to discussion instead}\adam{Feel free to move the part on Delphi to the related work section. It's a good idea.}

We measure the performance overhead of \capc in comparison to MP2ML (built on top of HE-transformer for nGraph), which is used in \capc. We measure the CPU, network (NET), and memory (MEM) utilization (\%) during execution of the MP2ML and \capc protocol on a CryptoNet-ReLU model with a mini-batch that contains only a single data item. Our micro-analysis of the performance, carried out using sar~\citep{sar}, is presented in Figures~\ref{fig:he-transformer-perf} and~\ref{fig:capc-perf} (with labels denoting the steps of the \capc protocol). %(in appendix). 
The trends are very similar and \capc incurs only a negligible additional resource usage (for example, only 2\% more CPU used on average). The workload is CPU bound and MP2ML runs only on CPUs (it does not support model inference on GPUs). We measure the utilization of all 20 cores in our experiment, network utilization out of 500 MB provided capacity, and the total memory usage on the server with 128 GB RAM. The network usage reaches its peaks during execution of ReLU and then MaxPool, where the intermediate feature maps have to be exchanged between the querying and answering parties for the computation via garbled circuits.

Overall, the additional features offered by \capc on top of MP2ML incur a low additional cost, which might enable its future applicability. %which is a promising result that might enable its practical use.

\begin{figure}[!htb]
   \begin{minipage}{0.49\textwidth}
     \centering %\includegraphics[width=1.0\linewidth]{figures/c_values.pdf}
     %\includegraphics[width=1.0\linewidth]{figures/c_values6.pdf}
     \includegraphics[width=1.0\linewidth]{graphs/performance-he-transformer2.pdf}
     \caption{\label{fig:he-transformer-perf} MP2ML (HE Transformer for nGraph).}
   \end{minipage}
   \hspace{\fill}
   \begin{minipage}{0.49\textwidth}
     \centering
    % \includegraphics[width=1.0\linewidth]{figures/hessian/highest_eigenvalues_CIFAR10.pdf}
    %\includegraphics[width=1.0\linewidth]{figures/hessian/highest_eigenvalues_histogram_data_len_1024_dataset_name_CIFAR-10_ver3.pdf}
    \includegraphics[width=1.0\linewidth]{graphs/performance-capc2.pdf}
    \caption{\label{fig:capc-perf} \capc (built on top of MP2ML).}
   \end{minipage}\hfill
\end{figure}




==> Contents/recycle_bin.tex <==
\subsection{Deep Learning}
\adam{If we need some more space later on, then we can shorten this subsection.}

Neural networks, as a family of highly expressive parameterized models, are capable of approximating arbitrarily complex continuous mappings from one domain to another by composing multiple layers of basic building blocks, such as linear convolutions and rectified linear units~\citep{glorot2011deep}. During the process of forward propagation, data points from the input domain are transformed by the operation defined in each layer in sequential order to produce their corresponding outputs. Meanwhile, the outputs of intermediate layers reveal a rich hierarchy of feature representations describing the inputs at different abstraction level, with upper layers capturing more abstract notions. Theoretical and empirical results \citep{telgarsky2016benefits,eldan2016power,vgg} validate the importance of deep feature hierarchy to the predictive power of neural networks, encouraging deeper model designs~\citep{resnet} and boosting research interests in deep learning.

To fit a deep neural network (DNN) with parameters $\theta$ to a training dataset $d = \{(x_{i}, y_{i})\}_{1 \leq i \leq N}$, we need to define an appropriate loss function $\mathcal{L}(\theta, d)$ that evaluates goodness of fit and then update $\theta$ in a way that minimizes $\mathcal{L}(\theta, d)$. Typically, $\mathcal{L}(\theta, d)$ is non-convex and highly non-linear in $\theta$, which makes it intractable to solve for the global minimum $\theta_{\ast} = \argmin_{\theta} \mathcal{L}({\theta}, d)$. Instead, we often settle for local minimums found by SGD-based optimization algorithms in practice. Precisely, the gradient of loss function $\nabla_{\theta} \mathcal{L}(\theta, d)$ is computed to iteratively update $\theta$ until the convergence is reached.



BELOW = put somewhere else

These often take the form of a decentralized learning algorithm. For instance, federated learning~\citep{konevcny2016federated} proposes to have participants help a central party train a model by sharing gradients: rather than send their data to the central party, each participant computes a model update on their local data and shares this update with the central party. While this provides confidentiality, it does not protect privacy because gradients shared still contain private information despite the data itself not being shared. To also preserve the participants' privacy, federated learning needs to be adapted to perform differentially private training. This is possible, but involves large datasets with billions of training points~\citep{mcmahan2017learning} since the data is not collected in a central location~\citep{chaudhuri2011differentially,abadi2016deep} to preserve confidentiality.

An algorithm preserves confidentiality when it does not reveal information an adversary is not authorized to access. Instead, an algorithm provides privacy when an adversary observing the algorithm's behavior is unable to infer any property of the training data which they did not already know of, as exemplified in the \textit{differential privacy} definition~\citep{dwork2006calibrating}. Put another way, confidentiality can be understood as preventing the explicit sharing of data whereas privacy limits implicit sharing of data. 

Furthermore, sharing gradients rather than data also inhibits the development of new model architectures.

Indeed, NN models can be prone to overfitting and may have incorrectly modeled different demographic groups\footnote{Samples in a dataset can be divided into a number of demographic groups based on various factors, such as class labels for classification tasks or feature attributes for general prediction tasks.} Our protocol allows the parties to gain access to a larger set of  high-quality samples that properly cover feasible regions of the learning task's input space. 

